SDSS IV MaNGA -- Metallicity and ionisation parameter in local star-forming galaxies from Bayesian fitting to photoionisation models

We measured gas-phase metallicity, ionisation parameter and dust extinction for 1795 representative local star-forming galaxies using integral field spectroscopy from the SDSS-IV MaNGA survey. We self-consistently derive these quantities by comparing observed line fluxes with photoionisation models using a Bayesian framework. We also present the first comprehensive study of the [SIII]$\lambda\lambda$9069,9532 nebular lines, which have long been predicted to be ideal tracers of the ionisation parameter. Unfortunately, we find that current photoionisation models substantially over-predict [SIII] lines intensity, while broadly reproducing other observed optical line ratios. We discuss how to nonetheless make use of the information provided by [SIII] lines by setting a prior on the ionisation parameter. Following this approach, we derive spatially-resolved maps and radial profiles of metallicity and ionisation parameter. The metallicity radial profiles are comparable with previous works, with metallicity declining toward the outer parts and a flattening in the central regions, in agreement with infall models of galaxy formation, that predict that spiral discs build up through accretion of material, which leads to an inside-out growth. On the other hand, ionisation parameter radial profiles are flat for low-mass galaxies, while their slope becomes positive as galaxy mass increases. However, the ionisation parameter maps we obtain are clumpy, especially for low-mass galaxies. Ionisation parameter is tightly correlated with the H$\alpha$ equivalent width [EW(H$\alpha$)], following a nearly universal relation, which we attribute to the change of the spectral shape of ionising sources due to ageing of HII regions. We derive a positive correlation between ionisation parameter and metallicity at fixed EW(H$\alpha$), in disagreement with previous theoretical works expecting an anti-correlation.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
